Multiphase Chemical Evolution in Elliptical Galaxies

The recent {\em ASCA} results show that the iron abundance of the X-ray gas of elliptical galaxies is less than the solar abundance ($Z_{\sun}$). The observed low iron abundance is inconsistent with the predictions of the previous chemical evolution models. In order to solve this problem, we present a simple model of chemical evolution for elliptical galaxies after the galactic wind period under the assumption that the gases ejected from stars do not mix with the circumferential gas. The ejected gas components evolve separately according to their birth time and origin. We have investigated their evolution qualitatively. The gas components originated from supernova remnant shells cool and drop out of the hot gas faster than the other components because of their high density and metal abundance. As a result, supernovae cannot heat the whole gas of the elliptical galaxies effectively, in contrary to the previous results. If the metal abundance of mass-loss gas is not uniform, the mass-loss gas with higher abundance also easily drops out and the average abundance can decrease. We believe that this is a hint of solving the low abundance problem.

==> tab1.tex <==
% TABLE1.TEX -- AASTeX sample table 1.

% The following gobbledygook is done so that this particular table
% paginates in a way that "looks nice" regardless of whether apjpt4
% or aj_pt4 styles are chosen.  The \tablebreak commands that appear
% after some of the lines force page breaks when the apjpt4 style is
% selected, but act simply as line delimiters for aj_pt4.

\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

% From here on, the file contains tabular data as an author might
% prepare it.

\begin{deluxetable}{ccccccccc}
%\tablewidth{33pc}
\tablewidth{0pc}
\tablecaption{Parameters of Models}
\tablehead{
\colhead{Model}          & \colhead{$M_{\rm g}(t_{0})$}      &
\colhead{SN rate}        & \colhead{$Z_{\rm ML}$}            &
\colhead{$n$}            & \colhead{$N_{\rm ML,H}$}          &
\colhead{$N_{\rm ML,L}$} & \colhead{$N_{\rm sh}$}            & 
\colhead{$N_{\rm cav}$}  
%\colhead{$Z$}            & \colhead{$Z_{\rm fit}$}           & 
%\colhead{$T_{\rm fit}$}  & \colhead{$N_{\rm H,fit}$}         &
%\colhead{[Fe/H]} 
\\
\colhead{}               & \colhead{($10^{10}\rm M_{\sun}$)} &
\colhead{(SNu)}          & \colhead{($Z_{\sun}$)}            &
\colhead{}               & \colhead{}                        &     
\colhead{}               & \colhead{}                        &
\colhead{}
%\colhead{($Z_{\sun}$)}   & \colhead{($Z_{\sun}$)}            &
%\colhead{(keV)}          & \colhead{($10^{21}\rm cm^{-2}$)}  &
%\colhead{ref}
}

\startdata
A1 & 0.65& 0.05& 1.0   & 133 & 91 & 91 & 10& 133 \nl
A2 & 0.65& 0.02& 1.0   & 138 & 33 & 33 &  7& 138 \nl
A3 & 0.65& 0.2 & 1.0   & 117 & 107& 107& 23& 117 \nl
A4 & 0.65& 0.05&1.5,0.5& 128 & 31 & 126& 25& 128 \nl
A5 & 0.65& 0.05&1.8,0.2& 124 & 37 & 124& 33& 124 \nl 
B1 & 0.9 & 0.05& 1.0   & 147 &\nodata&\nodata&\nodata&\nodata \nl
B2 & 0.9 & 0.02& 1.0   & 136 &\nodata&\nodata&\nodata&\nodata \nl
B3 & 0.9 & 0.2 & 1.0   & 161 &\nodata&\nodata&\nodata&\nodata \nl
B4 & 0.9 & 0.05&1.5,0.5& 213 & 21 & 49 & 12& 213 \nl
B5 & 0.9 & 0.05&1.8,0.2& 168 & 24 & 153& 21& 168 \nl
\enddata
\end{deluxetable}


==> tab2.tex <==
% TABLE2.TEX -- Sample table 2.

\begin{deluxetable}{ccccccccc}
%\tablewidth{33pc}
\tablewidth{0pc}
\tablecaption{Results of Fitting}
\tablehead{
\colhead{Model}          & \colhead{$L_{\rm X}$} &\colhead{Flux} & 
\colhead{Exposure}       & \colhead{$Z$}            & 
\colhead{$Z_{\rm fit}$}  & \colhead{$T_{\rm fit}$}  & 
\colhead{$N_{\rm H,fit}$}& \colhead{$\chi^{2}/$dof}   \\
\colhead{}               & \colhead{($10^{-40}\rm erg \: s^{-1}$)}
&\colhead{($10^{-12}\rm erg \:cm^{-2}\: s^{-1}$)}      &
\colhead{(ks)}            & \colhead{($Z_{\sun}$)}   & 
\colhead{($Z_{\sun}$)}   & \colhead{(keV)}          & 
\colhead{($10^{21}\rm cm^{-2}$)}  &  \\
}
\startdata
A1 & 24.6& 9.1 &     40  & 1.1 &    0.03 &     0.25 &  0.26   & 200/35 \nl
   &     &     &         &     &    0.65 &0.23, 1.0 &  0.08   & 32.4/32 \nl
A2 & 13.6& 5.1 &     40  & 1.0 &    0.10 &     0.32 &  0.11   & 48.1/27 \nl
   &     &     &         &     &    0.36 &0.33, 1.2 &  0.00   & 32.4/24\nl 
A3 &  1.5& 0.5 & \nodata & 2.3 & \nodata &  \nodata & \nodata & \nodata \nl
A4 & 0.3 & 0.1 & \nodata & 0.8 & \nodata &  \nodata & \nodata & \nodata \nl
A5 & 0.1 & 0.03& \nodata & 0.7 & \nodata &  \nodata & \nodata & \nodata \nl
B1 &\nodata&\nodata&\nodata&\nodata&\nodata&\nodata & \nodata & \nodata \nl
B2 &\nodata&\nodata&\nodata&\nodata&\nodata&\nodata & \nodata & \nodata \nl
B3 &\nodata&\nodata&\nodata&\nodata&\nodata&\nodata & \nodata & \nodata \nl
B4 & 8.6 & 3.2 &     80  & 0.8 &   0.04  &     0.41 &  0.20   & 133/42 \nl
   &     &     &         &     &   0.43  &0.40, 1.0 &  0.02   & 37.5/39 \nl
B5 & 1.5 & 0.6 & \nodata & 0.5 & \nodata &  \nodata & \nodata & \nodata \nl
\enddata
\end{deluxetable}

